Search for time-dependent $CP$ violation in $D^0 \to K^+ K^-$ and $D^0 \to \pi^+ \pi^-$ decays

A search for time-dependent violation of the charge-parity symmetry in $D^0 \to K^+ K^-$ and $D^0 \to \pi^+ \pi^-$ decays is performed at the LHCb experiment using proton-proton collision data recorded from 2015 to 2018 at a centre-of-mass energy of 13 TeV, corresponding to an integrated luminosity of 6 fb$^{-1}$. The $D^0$ meson is required to originate from a $D^*(2010)^+ \to D^0 \pi^+$ decay, such that its flavour at production is identified by the charge of the accompanying pion. The slope of the time-dependent asymmetry of the decay rates of $D^0$ and $\bar{D}^0$ mesons into the final states under consideration is measured to be $\Delta Y_{K^+ K^-} = (-2.3 \pm 1.5 \pm 0.3) \times 10^{-4}$, $\Delta Y_{\pi^+ \pi^-} = (-4.0 \pm 2.8 \pm 0.4)\times 10^{-4}$, where the first uncertainties are statistical and the second are systematic. These results are compatible with the conservation of the charge-parity symmetry at the level of 2 standard deviations and improve the precision by nearly a factor of two.

==> Makefile <==
# name of the main latex file (do not include .tex)
MAIN = main
MAIN_SUPPL = supplementary

# name of the target
TARGET = LHCb-PAPER-2020-045
TARGET_SUPPL = supplementary

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
	BUILDCOMMAND_SUPPL=rm -f $(MAIN_SUPPL).aux && $(LATEX) $(MAIN_SUPPL) && bibtex $(MAIN_SUPPL) && $(LATEX) $(MAIN_SUPPL) && $(LATEX) $(MAIN_SUPPL)
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
	BUILDCOMMAND_SUPPL=rm -f $(MAIN_SUPPL).aux && $(LATEX) $(MAIN_SUPPL) && bibtex $(MAIN_SUPPL) && $(LATEX) $(MAIN_SUPPL) && $(LATEX) $(MAIN_SUPPL) && dvips -z -o $(MAIN_SUPPL).ps $(MAIN_SUPPL) && ps2pdf $(MAIN_SUPPL).ps && rm -f head.tmp body.tmp
endif

# list of all source files
# TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
TEXSOURCES = appendix.tex main.tex Authorship_LHCb-PAPER-2020-045.tex body.tex my-symbols-def.tex title-LHCb-PAPER.tex acknowledgements.tex lhcb-symbols-def.tex preamble.tex $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)


TEXSOURCES_SUPPL = my-symbols-def.tex lhcb-symbols-def.tex preamble.tex supplementary.tex main.bib standard.bib LHCb-PAPER.bib $(wildcard *.bib)
FIGSOURCES_SUPPL = $(wildcard figs-supplementary/*$(FIGEXT))
SOURCES_SUPPL    = $(TEXSOURCES_SUPPL) $(FIGSOURCES_SUPPL)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)
OUTPUT_SUPPL = $(TARGET_SUPPL)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)
$(OUTPUT_SUPPL): $(MAIN_SUPPL)$(MAINEXT)
	cp $(MAIN_SUPPL)$(MAINEXT) $(OUTPUT_SUPPL)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

$(MAIN_SUPPL)$(MAINEXT): $(SOURCES_SUPPL) Makefile
	$(BUILDCOMMAND_SUPPL)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

supplementary: $(OUTPUT_SUPPL)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl *.toc $(MAIN)$(MAINEXT) $(MAIN_SUPPL)$(MAINEXT) $(MAIN).ps $(MAIN_SUPPL).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

